Q-caching: an integrated reinforcement-learning approach for caching and routing in information-centric networks

Content delivery, such as video streaming, is one of the most prevalent Internet applications. Although very popular, the continuous growth of such applications poses novel performance and scalability challenges. Information-centric networks put content at the center, and propose novel solutions to such challenges but also pose new questions on the interface between caching and routing. In this paper, building on top of Q-routing we propose a caching strategy, namely Q-caching, which leverages information that is already collected by the routing algorithm. Q-caching promotes content diversity in the network, reducing the load at custodians and average download times for clients. In stylized topologies, we show that the gains of Q-caching against state-of-the-art algorithms are significant. We then consider the RNP topology, and show that Q-caching performance is more flexible while competitive when compared against existing algorithms.

==> resumo.tex <==
\begin{resumo}
A distribuição de conteúdo é uma das aplicações mais prevalentes na Internet. Embora muito popular, o crescente aumento na demanda por tais aplicações traz novos desafios.  Redes orientadas a conteúdo, ao focarem no conteúdo como parte essencial da rede, buscam soluções para vários desafios mas também trazem novas perguntas, na fronteira entre roteamento e armazenamento de conteúdo.  Neste artigo, baseando-se no Q-routing, propomos uma nova política de armazenamento, que denominamos Q-caching.  Q-caching aproveita-se de informações que são oferecidas pelo Q-routing para promover diversidade de conteúdos na redes, o que se traduz em menor carga nos servidores e diminuição do tempo médio de download experimentados pelos clientes.  Em topologias simples, nós mostramos numericamente a superioridade do Q-caching em comparação com outros algoritmos propostos na literatura.  Na topologia da RNP, mostramos que o Q-caching é flexível no sentido de permitir que diferentes funções de utilidade sejam levadas em conta, e ao mesmo tempo competitivo quando comparado com  algoritmos concorrentes. 
\end{resumo}
